Learning to Learn Words from Visual Scenes

Language acquisition is the process of learning words from the surrounding scene. We introduce a meta-learning framework that learns how to learn word representations from unconstrained scenes. We leverage the natural compositional structure of language to create training episodes that cause a meta-learner to learn strong policies for language acquisition. Experiments on two datasets show that our approach is able to more rapidly acquire novel words as well as more robustly generalize to unseen compositions, significantly outperforming established baselines. A key advantage of our approach is that it is data efficient, allowing representations to be learned from scratch without language pre-training. Visualizations and analysis suggest visual information helps our approach learn a rich cross-modal representation from minimal examples. Project webpage is available at https://expert.cs.columbia.edu/

==> tables/pointing_both.tex <==
\begin{figure}
\begin{floatrow}
\capttabbox{%
\begin{tabular}{ c l r r r r}
\toprule
 && \multicolumn{2}{c}{\textbf{Ratio}} &     \\
 \cmidrule(lr){3-4}
 &&\textbf{1:1}&\textbf{2:1}& \multicolumn{1}{c}{\makecell{\textbf{Cost}}} \\ \midrule
& \multicolumn{1}{l|}{Chance}             & 13.5 &  8.7 & \multirow{3}{*}{-}  \\ 
& \multicolumn{1}{l|}{BERT (scratch) \cite{bert}}             &  36.5  & 26.3  &  \\ 
& \multicolumn{1}{l|}{BERT with Vision \cite{Chen2019} }   &  63.4  & 57.5  & \\ \midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{EXPERT}} & \multicolumn{1}{l|}{Isolated attn}               &  69.0  & 57.8  &$O(n)$\\
&\multicolumn{1}{l|}{Tgt-to-ref attn}                     &  71.0  & 63.2 &$O(n)$\\ 
&\multicolumn{1}{l|}{Via-vision attn}                      &  72.7  & 64.5  &$O(n)$\\ 
&\multicolumn{1}{l|}{\hspace{0.25cm}+ Input pointing}                     &  \textbf{75.0}  & \textbf{67.4}  &$O(n)$\\ 

&\multicolumn{1}{l|}{Full attn}                      &  \textbf{76.6}  & \textbf{68.4}  & $O(n^2)$  \\ \midrule
& \multicolumn{1}{l|}{BERT (pretrained) \cite{bert}}             &  53.4  & 48.8  &  \\ 
\bottomrule
\end{tabular}
}{%
\caption{\textbf{Acquiring New Words on EPIC-Kitchens:} We test our model's ability to acquire new words at test time. The difficulty of this task varies with the number of distractor examples in the reference set. We show top-$1$ accuracy results on both 1:1 and 2:1 ratios of distractors to positives. The rightmost column shows computational cost of the attention variant used.}%
\label{tbl:pting}%
}
\capttabbox{%
\begin{tabular}{ l | r r  }
\toprule
\textbf{Method} & \textbf{1:1} &  \textbf{2:1} \\ \midrule
Chance & 3.4 & 2.3 \\
BERT (scratch) & 31.6 & 25.7 \\
BERT with Vision \cite{Chen2019} & 32.1 & 26.8 \\
EXPERT (ours) & \textbf{69.3} & \textbf{60.9} \\ \midrule
BERT (pretrained) & \textbf{69.4} & \textbf{60.8} \\
\bottomrule
\end{tabular}
}{%
\caption{\textbf{Acquiring New Words on Flickr30k:} We run the same pointing experiments as in Table \ref{tbl:pting}, but on the Flickr30k dataset, which has more complex textual data. Here, chance is significantly lower, and our model significantly outperforms baselines. Due to its strong lexical acquisition policy, our model also performs as well as a text-only model pretrained on billions of tokens.}%
\label{tbl:pting_flickr}%
}
\end{floatrow}
\end{figure}

% \begin{table}[t]
% \begin{minipage}[t]{0.55\linewidth}
% \centering
% \begin{tabular}{ c l r r r r}
% \toprule
%  && \multicolumn{2}{c}{\textbf{Ratio}} &     \\
%  \cmidrule(lr){3-4}
%  &&\textbf{1:1}&\textbf{2:1}& \multicolumn{1}{c}{\makecell{\textbf{Cost}}} \\ \midrule
% & \multicolumn{1}{l|}{Chance}             & 13.5 &  8.7 & \multirow{3}{*}{-}  \\ 
% & \multicolumn{1}{l|}{BERT (scratch) \cite{bert}}             &  36.5  & 26.3  &  \\ 
% & \multicolumn{1}{l|}{BERT with Vision \cite{Chen2019} }   &  63.4  & 57.5  & \\ \midrule
% \multirow{5}{*}{\rotatebox[origin=c]{90}{EXPERT}} & \multicolumn{1}{l|}{Isolated attn}               &  69.0  & 57.8  &$O(n)$\\
% &\multicolumn{1}{l|}{Tgt-to-ref attn}                     &  71.0  & 63.2 &$O(n)$\\ 
% &\multicolumn{1}{l|}{Via-vision attn}                      &  72.7  & 64.5  &$O(n)$\\ 
% &\multicolumn{1}{l|}{\hspace{0.25cm}+ Input pointing}                     &  \textbf{75.0}  & \textbf{67.4}  &$O(n)$\\ 

% &\multicolumn{1}{l|}{Full attn}                      &  \textbf{76.6}  & \textbf{68.4}  & $O(n^2)$  \\ \midrule
% & \multicolumn{1}{l|}{BERT (pretrained) \cite{bert}}             &  53.4  & 48.8  &  \\ 
% \bottomrule
% \end{tabular}
% \caption{\textbf{Acquiring New Words on EPIC-Kitchens:} We test our model's ability to acquire new words at test time. The difficulty of this task varies with the number of distractor examples in the reference set. We show top-$1$ accuracy results on both 1:1 and 2:1 ratios of distractors to positives. The rightmost column shows computational cost of the attention variant used.}
% \label{tbl:pting} 
% \end{minipage}\hfill\begin{minipage}[t]{0.43\linewidth}
% \centering
% \begin{tabular}{ l | r r  }
% \toprule
% \textbf{Method} & \textbf{1:1} &  \textbf{2:1} \\ \midrule
% Chance & 3.4 & 2.3 \\
% BERT (scratch) & 31.6 & 25.7 \\
% BERT with Vision \cite{Chen2019} & 32.1 & 26.8 \\
% EXPERT (ours) & \textbf{69.3} & \textbf{60.9} \\ \midrule
% BERT (pretrained) & \textbf{69.4} & \textbf{60.8} \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Acquiring New Words on Flickr30k:} We run the same pointing experiments as in Table \ref{tbl:pting}, but on the Flickr30k dataset, which has more complex textual data. Here, chance is significantly lower, and our model significantly outperforms baselines. Due to its strong lexical acquisition policy, our model also performs as well as a text-only model pretrained on billions of tokens.}
% \label{tbl:pting_flickr}
% \end{minipage}
% \end{table}


